Small Turing universal signal machines

This article aims at providing signal machines as small as possible able to perform any computation (in the classical understanding). After presenting signal machines, it is shown how to get universal ones from Turing machines, cellular-automata and cyclic tag systems. Finally a halting universal signal machine with 13 meta-signals and 21 collision rules is presented.

==> Newcommand.tex <==





==> eptcsdata.tex <==
\providecommand{\eid}{7}

